Voiced-Aware Style Extraction and Style Direction Adjustment for Expressive Text-to-Speech

Recent advances in expressive text-to-speech (TTS) have introduced diverse methods based on style embedding extracted from reference speech. However, synthesizing high-quality expressive speech remains challenging. We propose SpotlightTTS, which exclusively emphasizes style via voiced-aware style extraction and style direction adjustment. Voiced-aware style extraction focuses on voiced regions highly related to style while maintaining continuity across different speech regions to improve expressiveness. We adjust the direction of the extracted style for optimal integration into the TTS model, which improves speech quality. Experimental results demonstrate that Spotlight-TTS achieves superior performance compared to baseline models in terms of expressiveness, overall speech quality, and style transfer capability.

==> Table/Ablation_hyperparameter.tex <==
\input{MAIN_Variables}

\begin{table}[!t]
\renewcommand{\arraystretch}{0.8}
\caption{Impact of hyperparameters $\lambda_x$ and $\lambda_y$. Natural and robust accuracy of ResNet-18 on PGD$^{20}$, PGD$^{100}$, and AA attacks on CIFAR-10 datasets with various hyperparameters combined with PGD adversarial training methods. The chosen hyperparameters are marked in bold.}
\centering
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{|c c||c|c|c|c|}
\hline
\rule{0pt}{8pt}
 $\lambda_x$ & $\lambda_y$ & Natural & PGD$^{20}$ & PGD$^{100}$ & AA \\ \hline
 \textbf{0.0001} & \textbf{0.0005} & \textbf{84.87} & \textbf{50.47} & \textbf{49.61} & \textbf{46.73} \\ \hline
 0.0002 & 0.0005 & 84.72 & 50.12 & 49.54 &  46.22 \\ 
 0.00005 & 0.0005 & 85.51 & 50.04 & 49.39 & 46.35 \\ \hline
 0.0001 & 0.001 & 84.23 & 50.18 & 49.57 &  46.19 \\ 
 0.0001 & 0.00025 & 85.33 & 50.09 & 49.41 & 46.30 \\ \hline
\end{tabular}%
}
\label{Ablation_hyperparameter}
\end{table}

==> appendices.tex <==
% \input{chapters/appendix_codes}

==> beginnings/acknowledgement.tex <==
This work was partly supported by the Institute of Information \& Communications Technology Planning \& Evaluation (IITP) grant funded by the Korea government (MSIT) (Artificial Intelligence Graduate School Program (Korea University) (No. RS-2019-II190079), Artificial Intelligence Innovation Hub (No. RS-2021-II212068), AI Technology for Interactive Communication of Language Impaired Individuals (No. RS-2024-00336673), and Artificial Intelligence Star Fellowship Support Program to Nurture the Best Talents (IITP-2025-RS-2025-02304828)).

==> beginnings/dedicationpage.tex <==
% 감사의 글 예시 페이지입니다.

% 감사합니다.

==> beginnings/enabstract.tex <==
\input{MAIN_Variables}

Recent advances in expressive text-to-speech (TTS) have introduced diverse methods based on style embedding extracted
from reference speech. However, synthesizing high-quality expressive speech remains challenging. We propose SpotlightTTS, which exclusively emphasizes style via voiced-aware style
extraction and style direction adjustment. Voiced-aware style
extraction focuses on voiced regions highly related to style
while maintaining continuity across different speech regions
to improve expressiveness. We adjust the direction of the extracted style for optimal integration into the TTS model, which
improves speech quality. Experimental results demonstrate
that Spotlight-TTS achieves superior performance compared to
baseline models in terms of expressiveness, overall speech quality, and style transfer capability. 


% \vspace*{\fill}
{\bf Keywords:}  Text-to-speech, style transfer, vector quantization

==> beginnings/krabstract.tex <==
최근 표현력 있는 음성 합성(TTS) 기술의 발전으로 참조 음성에서 추출한 스타일 임베딩 기반의 다양한 방법들이 제안되었습니다. 그러나 고품질의 표현력 있는 음성을 합성하는 것은 여전히 어려운 과제로 남아있습니다. 본 연구에서는 유성음 인식 스타일 추출과 스타일 방향 조정을 통해 스타일을 집중적으로 강조하는 Spotlight-TTS를 제안합니다. 유성음 인식 스타일 추출은 스타일과 높은 상관관계를 가진 유성음 영역에 집중하면서 표현력을 향상시키기 위해 서로 다른 음성 영역 간의 연속성을 유지합니다. 추출된 스타일의 방향을 조정하여 TTS 모델에 최적으로 통합함으로써 음성 품질을 개선합니다. 실험 결과는 Spotlight-TTS가 표현력, 전반적인 음성 품질, 스타일 전이 능력 측면에서 기존 모델들에 비해 우수한 성능을 달성함을 보여줍니다.

% \vspace*{\fill}
{\bf 주제어:} 음성합성, 스타일 전이, 벡터 양자화

==> beginnings/preface.tex <==
This dissertation is submitted for the degree of Master of Science in Artificial Intelligence at Korea University.
The research described herein was conducted under the supervision of Professor Seong-Whan Lee in the Department of Artificial Intelligence, Korea University. Part of this work has been presented at the Interspeech 2025. I was the lead investigator for the projects where I was responsible for all major areas of concept formation, data collection and analysis, as well as the majority of manuscript composition. Neither this, nor any substantially similar dissertation has been or is being submitted for any other degree, diploma, or other qualification at any other university.

% All of the work presented henceforth has been conducted in the \textit{Lab for Informatics, Communications, and Systems} at the Korea University, under the supervision of professor Sang Hyun Lee. The research described herein was conducted under the supervision of professor Sang Hyun Lee, between October 1998 and October 2001.
% It is to the best of my knowledge original, except where acknowledgments and references are made to previous work.

% Part of this thesis has been submitted as a conference paper and accepted for presentation in IEEE GLOBECOM 2022 Workshops.
% The corresponding information is as follows :\\% publication in the corresponding proceedings

% S. Kim, H. K. Kim, and S. H. Lee, ``Survey Propagation for Cell-Free Massive MIMO Pilot Assignment,'' in {\em Proc. IEEE Globecom Workshops (GC Wkshps), Rio de Janeiro, Brazil, Dec. 2022}, in press.\\

% While the project has been performed by my lead, there have been thankful contributions from several intellectuals. % responsible for the problem formulation, computational design of algorithm, major areas of concept formation, data collection and analysis, as well as manuscript composition.
% Professor Sang Hyun Lee is the supervisory author of the paper and has been involved throughout the project. 
% His insights and knowledge have motivated to employ a physical approach in this work.
% Hong Ki Kim has organized a simulation environment for the demonstration of our algorithm, and co-worked on manuscript edits and proofreading. Hong Ki Kim established a simulation environment for the verification of our proposed algorithm, and then worked together on editing and reviewing the manuscript.
% I sincerely appreciate their true support.

==> chapters/MAIN_Variables.tex <==
\renewcommand{\methodname}{STAARS}
\renewcommand{\weightcomponent}{class-specific multiplier}

==> chapters/formulation.tex <==
% \chapter{Pilot Assignment Problem}\label{section:formulation}

% The achievable rate for each user is damaged by the interference among pilot-sharing users. In this regard, the PA management is required constantly to ensure the network performance. While the pilot resources are repeatedly managed for each coherence interval, the large-scale channel parameters for some users are assumed to be preserved even if the interval is updated. In order to alleviate the computational loads, the latest assignments for those cases can leverage the  non-orthogonal PA task. 
% The initial setup policy is conducted so that the results of previous assignments for static users are maintained in the new PA.
% To this end, such users are preassigned with the same pilot sequence as the previous assignment, and it is assumed that $N_p$ of users are orthogonally preassigned to all of the pilot resources.

% \begin{figure}[!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/fig3-1_toyexample_preassign.eps}
%     \caption{An example of 6-user PA with preassignment.}%\vspace*{-.5em}
%     \label{fig:3.1}
% \end{figure}

% % \subsection{Pilot-Sharing}
% For ease of description, a simple example in Fig. \ref{fig:3.1} is considered where two pilots are assigned to six users and both are preassigned to user 1 and user 4, respectively.
% Let a set $\mathcal{P}_a$ be indices of preassigned users to which the $a$-th pilot sequence is dedicated, i.e., $\mathcal{P}_1 =\{1\}$  and $\mathcal{P}_2 =\{4\}$. The PA problem is characterized by a combinatorial optimization to select pilot-sharing groups that share the same pilot sequences as the preassigned users. 
% The PA solution is obtained so that the number of pilot-sharing users is as uniform as possible over pilot sequences. Since $K-N_p$ remaining users need the assignment, it is grouped into ${(K-N_{p})}/{N_{p}}$ members, and there are ${K-N_p \choose K/N_{p} -1}$ different feasible groups. Let $\mathcal{K}_{i}$ denote the $i$-th feasible group ($i=1,\ldots, {K-N_p \choose K/N_{p} -1}$). In the example, we have ${4 \choose 2}=6$ feasible groups, i.e., $\mathcal{K}_{1}=\{2,3\}, \dots, \mathcal{K}_{6}=\{5,6\}$. %toy example 그림 만들어서 설명하자
% % feasible group 중에는 같은 유저를 포함하는
% Since each user is assigned a single pilot, the feasible groups are selected so that the elements do not overlap in one solution.
% For the concrete indication of the PA, an integer variable $x_i$ is associated with the pilot sequence assigned to users in group $\mathcal{K}_i$. Thus, It holds that $x_i=a$ if the group $\mathcal{K}_i$ is matched with $a$-th pilot and $x_i=0$ otherwise. In addition, the corresponding state vector $\mathbf{x}=[x_1,\dots,x_{6}]$ is defined. Fig. \ref{fig:2_toy} shows the example for the case where $\mathcal{K}_1$ and $\mathcal{K}_6$ are used for PA among the feasible groups. The corresponding solution is  $\mathbf{x}=[1,0,0,0,0,2]$. % 솔루션이 유효하기 위해선 할당에 사용된 feasible group 간에 멤버 중복이 발생하지 않아야 한다.

% \begin{figure}[!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/fig2_toy_example}
%     \caption{The relationship among variables in a 6-user PA example.}%\vspace*{-.5em}
%     \label{fig:2_toy}
% \end{figure}

% Among the valid states, PA tasks are purposed to find the optimal solution that maximizes the network-wide utility such as sum-rate.
% A partial sum-rate denoted by $R_{i a}$ is defined corresponding to the pilot-sharing members if users in  $\mathcal{K}_i$ are assigned to the $a$-th pilot and given as
% \begin{equation}
%     {R}_{i a} \triangleq \sum_{k \in \mathcal{K}_i} R_{k} + \sum_{l \in \mathcal{P}_a} R_{l} \, .\label{eq:weight_rate}
% \end{equation}

% \section{Generic Formulation}

% % Where $i$ and $a$ belong to the set of indices of feasible groups $\mathcal{I}$ and pilot resources $\mathcal{A}$,
% % Each set of indices of feasible groups and pilot resources is denoted as $\mathcal{I}$ and $\mathcal{A}$, respectively.
% Let $\mathcal{I}$ denote the set of indices for feasible groups and $\mathcal{A}=\{1,\dots,N_\mathrm{p}\}$ be the set for pilot resources. the corresponding PA problem is formulated as
% \begin{subequations}
% \begin{align}
% \text{\textbf{(P1)}}\ \max_{\mathbf{x}} & \sum_{i \in \mathcal{I}} \sum_{a \in \mathcal{A}} {R}_{i a} \mathbbm{I}\left(x_{i}=a\right) &&\\
% \text{subject to~} & x_i \in \mathcal{A} \cup \{0\} \, ,~\forall i \in \mathcal{I} \, ,\\
% &\sum_{i \in \mathcal{I}}\mathbbm{I}\left(x_i=a\right)\leq 1 \, , ~\forall a \in \mathcal{A} \, , \label{eq:const_one} \\
% &\sum_{\mathclap{\ i^{\prime} \in \mathcal{N}(i)}} \mathbbm{I}\left(\left(x_i \neq 0\right) \land \left(x_{i^{\prime}} \neq 0 \right)\right)=0 \, , ~\forall i \in \mathcal{I} \, , \label{eq:const_neigbor}
% %&\mathbbm{I}\left(x_i \neq 0\right)+\mathbbm{I}\left(x_{i^{\prime}} \neq 0\right) \leq 1,~i^{\prime} \in \mathcal{N}(i), \forall i, 
% \end{align}
% \end{subequations}
% where $\mathbbm{I}(\cdot)$ is the indicator function that yields one if the input statement holds true and zero otherwise, $\land$ is the logical intersection, and $\mathcal{N}(i)$ is the set of neighborhoods of the $i$-th group, i.e., $\mathcal{N}(i) = \{i^{\prime}:\mathcal{K}_i \cap \mathcal{K}_{i^{\prime}} \neq \emptyset, i^{\prime} \neq i \}$. 
% The constraint in \eqref{eq:const_one} indicates that at most one group is allocated to each pilot. Furthermore, the constraint in \eqref{eq:const_neigbor} means that feasible groups containing the same users are not used simultaneously for a PA solution.
% % , since each user is assigned a single pilot rather than multiple pilots.
% % Furthermore, the constraint in \eqref{eq:const_neigbor} means that only a single pilot is assigned to each user.

% \section{Unconstrained Optimization Formulation}
% The constraints in \textbf{(P1)} are associated with the groups assigned to individual pilots. 
% This point of view motivates the introduction of a new function that considers the entire constraints. To represent them in an analytical way, a penalizing function for ${a}$-th pilot, $\mathcal{F}_{a}\left(\mathbf{x}\right)$, is defined to return a negative infinite value when the input vector $\mathbf{x}$ violates constraints related to \eqref{eq:const_one} and \eqref{eq:const_neigbor} as
% \begin{subequations}
% \begin{empheq}[left={\hspace*{-.6em}\mathcal{F}_{a}\left(\mathbf{x}\right)\triangleq\empheqlbrace}]{align}
%     {-\infty} &\ \text{ if } \textstyle\sum\limits_{i \in \mathcal{I}}\mathbbm{I}\left(x_{i}=a\right)>1 \, ,\label{eq:case_one}\\
%     %-\infty &{}\nonumber\\[-5pt]
%     {}&\ \text{ or } \exists i ~\text{s.t. } \textstyle\sum\limits_{\mathclap{\ i^{\prime} \in \mathcal{N}(i)}} \mathbbm{I}\left(\left(x_i \neq 0\right) \land \left(x_{i^{\prime}} \neq 0 \right)\right)\neq 0 \, ,\hspace*{-2em}\label{eq:case_neighbor}\\
%     0\ &\ \text{ otherwise} \, .
% \end{empheq}
% \end{subequations}
% %\begin{subequations}
% %\begin{numcases}{\mathcal{F}_{a}\left(\mathbf{x}\right)\triangleq }
% %    -\infty & if $\sum\limits_{i \in \mathcal{I}}\mathbbm{I}\left(x_{i}=a\right)>1$,\label{eq:case_one}\\[3pt]
% %    -\infty & if $\exists i ~\text{s.t. } \sum\limits_{\mathclap{\ i^{\prime} \in \mathcal{N}(i)}} \mathbbm{I}\left(\left(x_i \neq 0\right) \land \left(x_{i^{\prime}} \neq 0 \right)\right)\neq0$,\hspace*{-2em}\nonumber\\[-1em]\label{eq:case_neighbor}\\
% %    0 & otherwise.
% %\end{numcases}
% %\end{subequations}
% % Note that \eqref{eq:case_neighbor} corresponds to the case where $\mathcal{K}_{i}$ is assigned to the $a$-th pilot when any neighbor group of $\mathcal{K}_{i}$ is used to the assignment associated with \eqref{eq:const_neigbor}. The constraint in \eqref{eq:case_one} corresponds to the constraint in \eqref{eq:const_one}. However, the neighbor groups are not considered since \eqref{eq:case_neighbor} includes such a case.
% Note that the case \eqref{eq:case_one} is associated with the constraint in \eqref{eq:const_one}, but specifically focuses on the ${a}$-th pilot. The case \eqref{eq:case_neighbor} corresponds to that some neighboring groups are used in a PA solution so violating the constraint in \eqref{eq:const_neigbor}. 
% Likewise, a utility function $\mathcal{R}_i$ is defined to represent the weight for the objective function by the value of variable $x_i$ as
% % \begin{numcases}{\mathcal{R}_{i}\left(x_i\right)\triangleq }
% %     R_{i a} & if $x_i = a$, and $a \in  \{0, \cdots, N_\mathrm{p}\}$,\\
% %     0 & otherwise.
% % \end{numcases}
% \begin{equation}
%     \mathcal{R}_{i}\left(x_i\right) \triangleq \sum_{a \in \mathcal{A}}{R}_{i a} \mathbbm{I}\left(x_{i}=a\right).\label{rrr}
% \end{equation}%\vspace*{-.7em}

% An unconstrained optimization formulation from \textbf{(P1)}  is obtained from \eqref{rrr} as
% \begin{align}\label{eq:p1prime}
%     \text{\textbf{(P2)}}\ 
%     \max_{\mathbf{x}} &     \sum_{i \in \mathcal{I}} \mathcal{R}_i (x_i) 
%     + \sum_{a \in \mathcal{A}} \mathcal{F}_a(\mathbf{x}) \, .
%     % \text{subject to} & \nonumber \\
%     % &x_i \in [0, T], \ \forall i.
% \end{align}
% The optimal solution of (\textbf{P2}) is identical to that of (\textbf{P1}). Since this is factorized as a simple sum of utility functions and penalizing functions, this allows us to establish a distributed approach to solve the problem. 
% The optimal states are found locally by individual functions, and their information is exchanged for comparison with each other.
% The state variables are repeatedly corrected to deactivate all the penalizing functions and are expected to converge to a global solution that optimizes the total sum of the utility functions. % Some state variables that have inconsistent assignment are repeatedly corrected to be consistent over all functions and are expected to converge to a valid global solution that optimizing the total sum of the functions.
% In the next chapter, we presents an efficient solution for \textbf{(P2)} based on a cooperative consideration over a graphical representation of the overall optimization task.

==> chapters/numericalresults.tex <==
% \chapter{Numerical Results}\label{Results}

% % \begin{figure}
% %     \centering
% %     \includegraphics[width=\columnwidth]{figures/result.pdf}
% %     \caption{Simulation results} % in case resource per user lamda is 1.23 and 1.75 (a) cumulative distribution of sum rate with N=80 (b) sum rate versus the number of users
% %     \label{fig:results}
% % \end{figure}

% % 파라미터 셋업+비교스킴, 비교 내용 + 결과

% \section{Experimental Setup}
% This section presents numerical results to test the performance of the developed algorithm. A CF massive MIMO configuration is considered so that $M$ APs and $K$ users are equipped with a single antenna and randomly distributed over a $500\mathrm{m}\times500\mathrm{m}$ square area. The simulation region is wrapped around in order to mitigate the boundary effects \cite{2017versus}. 
% The heights of APs and users are set as $10$m and $1.5$m, respectively. The communication bandwidth of 20$\mathrm{MHz}$ and carrier frequency of $2\mathrm{GHz}$ are used. The normalized transmit SNR is set to $\omega=\bar{\omega}/\omega_{\text{noise}}$, with $\bar{\omega}=100 \mathrm{mW}$ and the noise power $\omega_{\text{noise}}=-92 \mathrm{dBm}.$ 
% The 3GPP Urban Microcell path loss model is used to set large-scale propagation conditions, where the shadow fading model is set to $z_{m k}\sim \mathcal{N}(1,\sigma_{\mathrm{sh}}^2)$ with $\sigma_{\mathrm{sh}}=4\mathrm{dB}$ \cite[Table B.1.2.1-1]{3GPP.36.814}.
% % {\color{red} The path loss and shadow fading models described in \cite{2017versus, 2022topological} are used to set large-scale propagation condition.} 
% % Without shadow fading "correlation"$.
% The length of the coherence interval $N_\mathrm{c}$ is taken as 200.
% We assume that the channels are constant during the coherence interval, and all users transmit with full power so that $\eta_k = 1$.

% %\textcolor{orange}{(K-means, topologic? 추가)}
% The proposed algorithm is compared with three existing PA schemes based on greedy algorithm \cite{2017versus}, K-means clustering \cite{2021structured}, and Hungarian algorithm \cite{2021Hungarian}.
% The greedy strategy repetitively identifies the pilot-user pair with the least user throughput and assigns a new pilot sequence to the identified user while fixing all other PA configurations. In K-means clustering based PA, all users are grouped by $N_\mathrm{p}$ members, then pilots are assigned orthogonally to users in each cluster. At this time, $\lceil K/N_\mathrm{p} \rceil$ centroids for the deployment of the APs are used for user clustering, and the centroids have been trained through the K-means clustering algorithm. On the other hand, Hungarian algorithm-based strategy execute the following tasks sequentially for each user: select $N_\mathrm{p}-1$ users with the highest proximity and conduct the bipartite matching for PA while the assignment of other users is fixed. 
% %%% fig(a)와 (b) 각각 내용을 문단별로 설명하자. K, T 규모,e.g. a CF massive MIMO configuration is considered so that $M=100$ APs and users ranging $15\leq K \leq 75$, 및 genetic 등 설명
% %The proposed algorithm is evaluated based on the initial setup policy described in Section \ref{section:formulation}. 
% In each simulation, $N_\mathrm{p}$ users are chosen at random and orthogonal pilots are preassigned to them so that PA is needed for the other $K-N_\mathrm{p}$ users.
% Note that pre-assignment for some users poses a risk of performance degradation instead of improving the PA complexity.
% For other benchmarks, we set up those to show full performance without pre-assignment.
% We evaluate the additional gain for SP framework with respect to Hungarian algorithm, K-means clustering, and greedy algorithm, respectively. The corresponding percentages are calculated based on the performance of each benchmark. 
% % 우리는 우리가 제안하는 알고리즘이 상술한 initial setup policy을 바탕으로 구동되었을 시의 성능을 검증하였다. 일부 유저의 파일럿 할당을 고정하는 전략은 PA의 복잡도를 개선하는 대신에 성능 하락을 감수한다는 점을 유의하라. 다른 벤치마크의 경우 별도의 pre-assignment 없이 기존에 보고된 성능을 보이도록 설정하였고 이를 우리의 제안과 비교하였다.

% \section{Results and Discussions}

% % \begin{figure}[!t]
% %     \centering
% %     \includegraphics[width=\columnwidth]{figures/fig4_results}
% %     \caption{Simulation results in case $M=100$ and $K/N_{\mathrm{p}}=3$. (a) CDF of system throughput where $K=45$. (b) Average system throughput versus number of users.}
% %     \label{fig:results}
% % \end{figure}

% \begin{figure}[]
%     \centering
%     \includegraphics[width=.7\textwidth]{figures/fig5-1_results_CDF.eps}
%     \caption{Cumulative distribution function of system throughput where $K=45, M=100, N_{\mathrm{p}}=15$.}
%     \label{fig:5-1}
% \end{figure}

% Fig. \ref{fig:5-1} illustrates the cumulative distribution function of the system throughput in uplink with $M=100$, $K=45$, and $N_\mathrm{p}=15$. 
% The proposed algorithm, SP, outperforms other benchmarks constantly over the simulation, thus indicating that the pilot contamination is effectively mitigated. 
% The average system throughput obtained by SP is about 744$~\mathrm{Mbps}$, which corresponds to the improvement over compared schemes by $2\%$, $5\%$, and $10.3\%$ respectively.
% %The SP framework enhances the average system throughput by $2\%$, $5\%$, and $10.3\%$ with respect to Hungarian algorithm, K-means clustering, and greedy algorithm, respectively. %In particular, only $39\%$, $26\%$, and $13\%$ can meet the median performance of the SP framework, respectively.
% % This indicates that SP-based solution is more successful at searching all solutions of feasible PA configuration spaces than the existing schemes.
% %This indicates that the SP framework can explore optimal PA solutions over existing performance even under pre-assignment conditions. %In addition, it also shows performance advantages in addition to reinforcing the sustainability.
% In addition, a popular metric for PA is the network throughput for the worst $5\%$ PA configurations \cite{2021structured, 2021Hungarian}.
% SP obtains the value of 657$~\mathrm{Mbps}$, and this amounts to $3\%$, $6\%$, and $13\%$ improvement over others, respectively.
% Thus, the population of low throughput users is decreased by the proposed method.

% \begin{figure}[]
%     \centering
%     \includegraphics[width=.7\textwidth]{figures/fig5-2_results_avg.eps}
%     \caption{Average system throughput versus number of users where $K\in\{15,30,45,60,75\}, M=100, N_{\mathrm{p}}=15$.}
%     \label{fig:5-2}
% \end{figure}
% Fig. \ref{fig:5-2} depicts the average system throughput where $M=100$ and $K\in\{15, 30, 45, 60, 75\}$. 
% The number of users per orthogonal pilot resources, $K/N_\mathrm{p}$, is fixed to $3$.
% For large user populations, the system throughput growth under all PA strategies attenuates due to the additional beamforming uncertainty and user interference from the network congestion. 
% At the largest population of $K=75$, the SP framework results about 907$~\mathrm{Mbps}$ then outperforms Hungarian algorithm, K-means clustering, and greedy strategies, respectively, by $1\%$, $4\%$, and $9\%$. This shows the robustness to the network congestion with respect to benchmarks. 

% The SP approach is suited to optimize corresponding tasks for network throughput maximization from the advantage achieved by organizing the PA task from a group-wise matching framework. This allows the achievable rate to be directly utilized in network management. Through the developed algorithm, the PA operation can be configured to explore the solution space of the PA efficiently.

==> chapters/proposedapproach.tex <==
% \chapter{Distributed Algorithm via Survey Propagation}

% It is noted that the PA problem inherits a unique nature that states interactively constrain each other, thus incurring many local solutions that significantly differ from the optimum. This corresponds to so-called {\em replica symmetry breaking} phenomenon in the field of statistical physics \cite{mezard1987spin}. 
% The SP \cite{2005survey} approach is investigated to tackle this challenge induced by such property. 
% %This is originally investigated in the field of statistical physics. 
% From the analogy of the PA solution space with the formation of stable interaction relationships among variables, this approach can be exploited to characterize an efficient distributed solution \cite{2016beyound}. To be precise, the central peak-point probabilities of the PA contained in a cluster of the local optimal solutions are found by implementing a distributed search algorithm via message-passing techniques \cite{2001factor,2007affinity}. Therefore, individual users may be able to participate in obtaining computationally demanding solutions. A detailed description of the strategy is presented in the following sections.

% \begin{figure}[!]
%     \centering
%     \includegraphics[width=\columnwidth]{figures/fig3_factor_graph}
%     \caption{Graphical representation for pilot assignment problem. (a) Factor graph model for \textbf{(P2)}. (b) Two types of messages between $\mathcal{F}_a$ and $x_i$.}
%     \label{fig:3_factor}
% \end{figure}

% \section{Graphical Representation}
% To derive the corresponding message-passing based distributed algorithm, the structure of a graphical model that facilitates the understanding of the problem structure is necessarily considered. 
% Fig. \ref{fig:3_factor}(a) illustrates a factor graph model \cite{2001factor} associated with the toy example. 
% Note that if the group $\mathcal{K}_1$ is used for assignment, it limits the groups in $\mathcal{N}(1)$ unused. While the use of $\mathcal{K}_1$ constrains the states of corresponding neighbor groups, other states are not determined but are prohibited from assigning the same pilot with $\mathcal{K}_1$.
% % In a valid PA solution with $x_1 = 1, x_6 = 2,$ and $x_i=0$ for $i\in\{2,3,4,5\}$, penalizing functions becomes zero, and two utility function take the outputs of $R_{1,1}$ and $R_{6,2}$, respectively.

% \section{Derivation of Algorithm}

% \subsection{Design Principles for Computation}
% According to generic message-passing computational rules \cite{2001factor}, the tendency for the allocation of the $a$-th pilot to group $\mathcal{K}_i$ in optimal states are characterized by messages exchanged between node $x_i$ and node $\mathcal{F}_a$. To this end, two different types of messages are defined, respectively, as shown in Fig. \ref{fig:3_factor}(b): $\rho_{i a}(x_i=x)$, a message transferred from $x_i$ to $\mathcal{F}_a$ informing how evident the value of $x_i$ can take on a value of $x$, and $\alpha_{i a}(x_i=x)$, a message sent from $\mathcal{F}_a$ to $x_i$ representing how preferable the value of $x_i=x$ is to satisfy the constraint enforced by the factor function $\mathcal{F}_a$.
% Under equilibrium states, both messages necessarily represent certain relationships between group $\mathcal{K}_i$ and $a$-th pilot is given according to the state of $x_i$ to maximize unconstrained formulation (\textbf{P2}) as
% \begin{align}
%     \rho_{i a}(x_i) = & ~\mathcal{R}_{i}(x_i) + \sum_{b \neq a} \alpha_{i b}(x_i) \, ,\label{eq:def_rho(x)}\\%[-.3em]
%     \alpha_{i a}(x_i) = & \max_{\mathbf{x}\backslash\{x_i\}}\Big(\mathcal{F}_a (\mathbf{x})+\sum_{j \neq i}\rho_{j a}(x_j)\Big) \, .\label{eq:def_alp(x)}
% \end{align}%\\[-.7em]
% Thus, $\rho_{i a}(x_i)$ and $\alpha_{i a}(x_i)$ take the values associated with the maximal objective when  group $\mathcal{K}_i$ is assigned to the $a$-th pilot. %In particular, while $\rho_{i a}(x_i)$ evaluates $x_i$'s allocation state, $\alpha_{i a}(x_i)$ searches optimal system state given $x_i$'s state.
% % weight function의 출력의 합을 최대화 하는 조합을 고려하는 와중에, penalizing 함수에 의해 system state에 가해지는 strict condition을 유의할 필요가 있음.

% %%%%%%%%%%%책갈피: fig3

% However, there may exist too many states of a PA task that slightly differ from optimal state $\mathbf{x}$ and take corresponding objective values very close to the optimum. 
% In order to control all these assignments collectively, a basic principle of handling combinatorial optimization with the SP framework is applied by introducing multiple possible states for individual discrete variables, representing {\em chosen}, {\em unchosen}, and {\em undetermined}. In the PA task, the state of an individual variable $x_i$ imposed by the constraint $\mathcal{F}_a$ can be categorized into three types: {\em assigned}, {\em idle}, and {\em elsewhere}. If $x_i = a$, any group that shares members with $\mathcal{K}_i$ becomes idle, and no other group is assigned to the $a$-th pilot. If $x_i = 0$, which means that $\mathcal{K}_i$ is idle, other groups do not care about it and go into the so-called don't-care state\cite{2005survey}.
% If $x_i \notin \{0, a\}$, which is associated with the elsewhere state, only the neighbor groups of $\mathcal{K}_i$ are restricted to being idle. % which is associated with elsewhere state, that only restrict the neighbor group of $\mathcal{K}_i$ idle state.
% %The elsewhere state is similar with the don't care state that many possible states is involved in both states. 

% To consolidate the relationship among these three states, three different types of messages are defined, i.e., %derivation of messages corresponding both Eq.\eqref{eq:def_rho(x)} and Eq.\eqref{eq:def_alp(x)} is available. While the messages about first two state, assigned and idle state, are 
% $\{\rho_{i a}^{(a)}, \alpha_{i a}^{(a)}\}$ and $\{\rho_{i a}^{(0)}, \alpha_{i a}^{(0)}\}$ along with new messages associated with elsewhere state, $\{\rho_{i a}^{(*)}, \alpha_{i a}^{(*)}\}$. 
% % The definition is given by
% % \begin{align}
% %     \rho_{i a}(*) \triangleq& \max_{x_i \notin \{0,a\}}\Big(\mathcal{R}_{i}(x_i) + \sum_{b \neq a} \alpha_{i b}(x_i)\Big),\label{eq:def_rho(else)}\\
% %     \alpha_{i a}(*) \triangleq& \max_{x_i \notin \{0,a\}} \max_{\ \mathbf{x}\backslash\{x_i\}} \Big(\mathcal{F}_a (\mathbf{x})+\sum_{j \neq i}\rho_{j a}(x_j)\Big).\label{eq:def_alp(else)}
% % \end{align}
% % While there are too many possible states corresponding to vector $x$, the quantization can be adopted, one of the strategy for establishing survey propagation\cite{2016beyound}. We quantize the set of messages $\{\rho_{i a}, \alpha_{i a}\}$ into three newly defined states; $\{\rho_{i a}(a), \alpha_{i a}(a)\}$ denotes the messages when $\mathcal{K}_i$ is assigned to $a$-th pilot such that $x_i = a$, $\{\rho_{i a}(0), \alpha_{i a}(0)\}$ denotes the messages when $\mathcal{K}_i$ is not used such that $x_i = 0$, and $\{\rho_{i a}(*), \alpha_{i a}(*)\}$ denotes the messages when $\mathcal{K}_i$ is assigned elsewhere such that $x_i \notin \{0,a\}$. The first two types of messages are equivalent to predefined messages 
% % where $x_i=a$ and $x_i=0$ respectively. The last type of messages are given by

% \subsection{Messages for Assigned States}

% If $x_{i}=a$, the message $\rho_{ia}(x_{i})$ is computed as follows.
% \begin{equation}
%     \rho_{ia}(a) = \mathcal{R}_{i}(a) + \sum_{b \neq a} \alpha_{i b}(a) = R_{i a} + \sum_{b \neq a} \alpha_{i b}(a) \, .
% \end{equation}
% Since the group $\mathcal{K}_{i}$ is assigned elsewhere from the $b$-th pilot such that $b \neq a$,
% \begin{equation}
%     \rho_{i a}^{(a)} = R_{i a}+\sum_{b \neq a} \alpha_{i b}^{(*)} \, .
% \end{equation}

% In the same case, the message $\alpha_{ia}(x_{i})$ is computed as follows.
% \begin{equation}
%     \alpha_{i a}(a) = \max_{\mathbf{x}\backslash\{x_i\}}\Big(\mathcal{F}_a (\mathbf{x})+\sum_{j \neq i}\rho_{j a}(x_j)\Big) \, .
% \end{equation}
% To avoid the penalizing function $\mathcal{F}_a$ returns negative infinity, all of the other state variables in $\mathbf{x}$ are prohibited to be $a$. The assigned message $\alpha_{i a}^{(a)}$ is then given by
% \begin{equation}
%     \alpha_{i a}^{(a)} = ~\sum_{\mathclap{i^{\prime} \in \mathcal{N}(i)}} \rho_{i^{\prime} r}^{(0)}
%     + \; \sum_{\mathclap{i^{\prime \prime} \in \mathcal{N}(i)^{c}\backslash \{i\}}} \max\Big(\rho_{i^{\prime \prime} r}^{(0)},\rho_{i^{\prime \prime} r}^{(*)}\Big) \, .
% \end{equation}

% \subsection{Messages for Idle States}

% If $x_{i}=0$, the message $\rho_{ia}(x_{i})$ is computed as follows.
% \begin{equation}
%     \rho_{ia}(0) = \mathcal{R}_{i}(0) + \sum_{b \neq a} \alpha_{i b}(0) = \sum_{b \neq a} \alpha_{i b}(0) \, .
% \end{equation}
% The corresponding idle message is straightforwardly given as follows, although the message $\alpha_{i a}^{(0)}$ is not.
% \begin{equation}
%     \rho_{i a}^{(0)} = ~\sum_{b \neq a} \alpha_{i b}^{(0)} \, .
% \end{equation}

% To compute the idle message $\alpha_{i a}^{(0)}$, we divide the idle state into two cases.
%     \begin{itemize}
%         \item \textbf{$a$-th pilot is utilized anyway:}\\
%         There is only one $j \neq i \text{ s.t. } x_{j}=a$,\\
%         then $x_{j^{\prime}}=0 \text{ for } j^{\prime} \in (N(j)\backslash \{i\}) \text{ and } x_{j^{\prime \prime}} \neq a \text{ for } j^{\prime \prime} \notin (N(j)\cup\{i\})$.
%         \item \textbf{$a$-th pilot is not used for the uplink training:}\\
%         $\nexists j \neq i \text{ s.t. } x_{j}=a$.
%         % $x_{\hat{i}}=0, \forall \hat{i} \neq i$.
%     \end{itemize}
% Since the message $\alpha_{i a}^{(0)}$ returns the maximum value among these cases, it is given by
% \begin{equation}
%     \alpha_{i a}^{(0)} = \max\begin{cases}
%         \ \max\limits_{j \neq i} \bigg(
%             \rho_{j a}^{(a)} + \quad \displaystyle\sum\limits_{\mathclap{{j}^{\prime} \in \mathcal{N}({j})\backslash \{i\}}} \rho_{{j}^{\prime} a}^{(0)} \ + \quad \sum\limits_{\mathclap{{j}^{\prime \prime} \in \mathcal{N}({j})^{c}\backslash\{{i, j}\}}} \quad \max\Big(
%                 \rho_{{j}^{\prime \prime} r}^{(0)}, \ \rho_{{j}^{\prime \prime} r}^{(*)}
%                 \Big)
%         \bigg)\ ,\\[2em]
%         \ \displaystyle\sum\limits_{j \neq i} \max \Big(\rho_{j a}^{(0)}, \rho_{j a}^{(*)}\Big)\ .
%     \end{cases}\label{eq:alpha_idle}
% \end{equation}

% \subsection{Messages for Elsewhere States}

% For representing a number of elsewhere states, we pick the maximum value of $\rho_{ia}(x_{i})$ and $\alpha_{ia}(x_{i})$, while $x_{i} \notin \{0,a\}$, respectively. The message $\rho_{i a}^{(*)}$ is then given by
% \begin{equation}
%     \rho_{i a}^{(*)} = ~\max_{b \neq a} \Big(R_{i b}+\alpha_{i b}^{(b)}
%     +\sum_{\mathclap{s \notin \{a, b\}}} \alpha_{i s}^{(*)}\Big) \, .
% \end{equation}

% We divide the idle state into two cases as same as $\alpha_{i a}^{(0)}$ to compute the idle message $\alpha_{i a}^{(*)}$, but the states of neighbor groups are limited to be idle in both of cases. Remainer descriptions of each case are as follows.
%     \begin{itemize}
%         \item \textbf{$a$-th pilot is utilized anyway:}\\
%         There is only one $j \notin (\mathcal{N}(i)\cup\{i\}) \text{ s.t. } x_{j}=a$,\\
%         then $x_{j^{\prime}}=0 \text{ for } j^{\prime} \in (N(i)\cup N(j)) \text{ and } x_{j^{\prime \prime}} \neq a \text{ for others}$.
%         \item \textbf{$a$-th pilot is not used for the uplink training:}\\
%         There is no state variable $x_{j}$ such that $x_{j}=a$.
%         % $x_{\hat{i}}=0, \forall \hat{i} \neq i$.
%     \end{itemize}
% Note that if $j \notin \mathcal{N}(i)$, $i \notin \mathcal{N}(j)$. The corresponding message is given by
% \begin{align}
%     \alpha_{i a}^{(*)} =& \sum\limits_{i^{\prime} \in \mathcal{N}(i)} \rho_{i^{\prime} a}^{(0)}\nonumber\\
%     &+ \max \begin{cases}
%     ~\max\limits_{j\in \mathcal{N}(i)^{c}\backslash \{i\}}\bigg(
%             \rho_{j a}^{(a)} + \ \displaystyle\sum\limits_{\mathclap{j^{\prime} \in \mathcal{N}(j) \backslash \mathcal{N}(i)}} \rho_{j^{\prime} a}^{(0)} \quad\;  + \quad\;  \sum\limits_{\mathclap{j^{\prime \prime} \in \mathcal{N}(j)^{c}\backslash(\{i\} \cup \mathcal{N}(i))}} \quad \max\Big(\rho_{j^{\prime \prime} a}^{(0)}, \rho_{j^{\prime \prime} a}^{(*)}\Big)
%         \bigg)\ , \\[2em]
%         \quad\;\
%         \displaystyle\sum\limits_{\mathclap{i^{\prime \prime} \in \mathcal{N}(i)^{c}\backslash \{i,j\}}} \max\Big
%             (\rho_{i^{\prime \prime} a}^{(0)},\ \rho_{i^{\prime \prime} a}^{(*)}
%         \Big)\ .
%     \end{cases}\label{eq:alpha_else}
% \end{align}

% \section{Rules for Message Update and Decision}

% The message-passing algorithm is conducted to collect the information of optimality that is encoded as aforementioned descriptions.
% Upon convergence of the messages, The decision of the value for $x_i$ is made using
% \begin{align}
% \tilde{b}_{i a} \triangleq& \ (\rho_{i a}^{(a)} - \rho_{i a}^{(0)}) + (\alpha_{i a}^{(a)} - \alpha_{i a}^{(0)})\, ,\\
% \bar{b}_{i a} \triangleq& \ (\rho_{i a}^{(a)} - \rho_{i a}^{(*)}) + (\alpha_{i a}^{(a)} - \alpha_{i a}^{(*)})\, .
% \end{align}
% If group index $a$ is found with possible $\max_{a} \tilde{b}_{i a}$, the $i$-th users combination is assigned the $\hat{x}_i$-th pilot resource, which is given by $\hat{x}_{i}=\arg\max_{ a} \bar{b}_{i a}$. Otherwise, the $i$-th users combination is released idle. 

% Note that the finally used forms of the messages are only two measures, difference between assigned state and idle state ($\{\rho_{i a}^{(a)} - \rho_{i a}^{(0)},~\alpha_{i a}^{(a)} - \alpha_{i a}^{(0)}\}$), difference between assigned state and elsewhere state ($\{\rho_{i a}^{(a)} - \rho_{i a}^{(*)},~\alpha_{i a}^{(a)} - \alpha_{i a}^{(*)}\}$). 
% While the compactness of the message exchange is essential, it is sufficient to make decisions by the compressed forms of messages that are reduced from three to two types. The corresponding measures can be defined and calculated, respectively, as %To make the expression shortly, part of the notation is shown in superscript, i.e. $\rho_{i a}^{(a)}=\rho_{i a}(a)$. The results are given as 

% \begin{align}
%     \tilde{\rho}_{i a} \triangleq& ~\rho_{i a}^{(0)} - \rho_{i a}^{(*)}= \sum\limits_{b \neq a}\left(\tilde{\alpha}_{i b} - \bar{\alpha}_{i b}\right)- \max_{ b \neq  a} \left(R_{i b}-\bar{\alpha}_{i b}\right),\nonumber\\[-1.4em]\label{eq:rho_tilde}\\
%     \bar{\rho}_{i a} \triangleq& ~\rho_{i a}^{(a)} - \rho_{i a}^{(*)}= R_{i a} - \max_{ b \neq  a} \left(R_{i b}-\bar{\alpha}_{i b}\right),\label{eq:rho_bar}\\%\\[10pt]
%     \tilde{\alpha}_{i a} \triangleq& ~\alpha_{i a}^{(0)} - \alpha_{i a}^{(a)}\nonumber\\%\text{ \textcolor{red}{부호 바꿔서 baseline을 통일시키기} }
%     =&  \bigg[\max\limits_{j \neq i}\Big(
%         \bar{\rho}_{j a} - \left[\tilde{\rho}_{j a}\right]^{+}
%         + \ \sum\limits_{\mathclap{ j^{\prime} \in \mathcal{N}({j})\backslash\{i\} }} \left[\tilde{\rho}_{j^{\prime} a}\right]^{-}
%         \Big)
%         \bigg]^{+}
%         - \sum\limits_{\mathclap{ i^{\prime} \in \mathcal{N}(i) }} \left[\tilde{\rho}_{i^{\prime} a}\right]^{-},\label{eq:alp_tilde}\\
%     \bar{\alpha}_{i a} \triangleq& ~\alpha_{i a}^{(*)}-\alpha_{i a}^{(a)}\nonumber\\
%     =& \bigg[
%         \max\limits_{{j}\in \mathcal{N}(i)^{c}\backslash \{i\} }\Big(
%         \bar{\rho}_{{j} a} - \left[\tilde{\rho}_{{j} a}\right]^{+}
%         + \ \sum\limits_{\mathclap{ {j}^{\prime} \in \mathcal{N}({j}) \backslash \mathcal{N}(i) }}{\left[\tilde{\rho}_{{j}^{\prime} a}\right]^{-}}
%         \Big)\bigg]^{+},\label{eq:alp_bar}
% \end{align}
% where $[\ \cdot \ ]^{+}=\max(0,\ \cdot\ ), \ [\ \cdot\ ]^{-}=\min(0,\ \cdot \ )$. Then the decision variables are caculated as followings.

% \begin{align}
% \tilde{b}_{i a}=&\ (\bar{\rho}_{i a}-\tilde{\rho}_{i a}) - \tilde{\alpha}_{i a} \, , \label{eq:b_tilde}\\
% \bar{b}_{i a}=&\ \bar{\rho}_{i a} - \bar{\alpha}_{i a}  \, . \label{eq:b_bar}
% \end{align}

% Algorithm 1 summarizes the overall SP-based distributed algorithm, where individual message update computations can be handled by individual users and tentative decisions are made by the CPU interconnected to APs. 

% \begin{algorithm}[!t]\label{alg:PA1}
%     \setstretch{1.2}
%     \caption{Distributed PA algorithm}
%     \begin{algorithmic}[1]
%     \renewcommand{\algorithmicrequire}{\textbf{Input:}}
%     \renewcommand{\algorithmicensure}{\textbf{Output:}}
%     \REQUIRE Partial sum-rate $\{R_{i a}\}$ for all $(i, a)$ in \eqref{eq:weight_rate}.
%     \ENSURE  Pilot indices of all users $\{x_i\}$
%     \STATE \textit{Initialization} : Set $\tilde{\alpha}^{[1]}_{i a} = 0$, and $\bar{\alpha}^{[1]}_{i a} = 0$ for all $(i,r)$ and $t \gets 1$.
%     \\\textbf{repeat}
%     \\\quad \textit{Message updates}
%     \STATE \qquad Update $\tilde{\rho}^{[t]}_{i a}$ and $\bar{\rho}^{[t]}_{i a}$ using \eqref{eq:rho_tilde} and \eqref{eq:rho_bar}, respectively.
%     \STATE \qquad Update $\tilde{\alpha}^{[t+1]}_{i a}$ and $\bar{\alpha}^{[t+1]}_{i a}$ using \eqref{eq:alp_tilde} and \eqref{eq:alp_bar}.
%     \\ \quad \textit{Tentative decision}
%     \STATE \qquad Evaluate $\tilde{b}_{ia}$ and $\bar{b}_{ia}$ using \eqref{eq:b_tilde} and \eqref{eq:b_bar}.
%     \STATE \qquad \textbf{if} ($\max_{a} \tilde{b}_{i a}>0$) \textbf{then} ${x}_{i} \gets \arg\max_{a} \bar{b}_{i a}$.
%     \STATE \qquad \textbf{else} ${x}_{i} \gets 0$.
%     \\ %\qquad \textbf{end if}
%      \STATE \quad \textit{Increment} : $t \gets t+1$.
%     \\\textbf{until} Convergence of all messages
%     \RETURN Allocate pilot according to $\{x_i\}$. 
%     \end{algorithmic} 
% \end{algorithm}

==> chapters/systemmodel.tex <==
% \chapter{Cell-Free Massive MIMO System}

% \begin{figure}[!]
%      \centering
%      \includegraphics[width=\textwidth]{figures/fig1_system_model}
%      \caption{Uplink transmission in cell-free massive MIMO system.}%\vspace*{-.5em}
%      \label{fig:1}
% \end{figure}

% % 우리는 \cite{2017versus, 2021structured, 2021Hungarian}에서 고려된 모델을 참고하여 시스템모델을 상정하였으며, 우리의 주제에 집중하기 위해 상황의 부수적 요인을 간소화시키는 몇가지 가정을 세팅하였다.
% A CF massive MIMO system consisting of $M$ APs and $K$ users ($K\leq M$), all equipped with a single antenna, is considered. Each user is served simultaneously by multiple APs operating with the shared radio resource. The coherence intervals of all channels are thus defined as the product of the coherence time and bandwidth. Individual APs are connected to a central processing unit (CPU) via fronthaul that provides error-free and infinite capacity links for straightforward focus on the PA operation.
% %The CPU is responsible for the control for them.

% %We assume that the fronthaul connection is perfect so that offer error-free and infinite capacity to the CPU, and channels are constant during the coherence interval. 
% % We note that our system model is simplified version of general CF massive MIMO in \cite{2017versus} to concentrate on our main topic, PA optimization. 

% This work mainly considers the uplink transmission since there is no need for downlink pilot training \cite{2017versus} and the channel reciprocity allows a straightforward extension to the downlink transmission \cite{2021structured}. In the uplink transmission operating in a time division duplex manner, a coherence interval, with its resource length $N_\mathrm{c}$, is divided into two phases: the uplink pilot training and the uplink payload transmission. During the first training phase of length $N_\mathrm{p}$, users transmit dedicated pilot sequences to APs, and APs attempt to estimate the user channel states. In the second phase of length $N_\mathrm{c}-N_\mathrm{p}$, the uplink signals are detected with those estimates. 

% \section{Uplink Training}

% Let $ \boldsymbol{\varphi}_{k} \in \mathbb{C}^{N_\mathrm{p} \times 1}$ be the unit norm pilot sequence used by $k$-th user, where $N_\mathrm{p}$ of orthogonal pilot sequences are available. The channel coefficient between the $k$-th user and the $m$-th AP during a coherence interval, denoted as $g_{m k}$, is defined by the small-scale fading $h_{m k}$ and large-scale fading $\beta_{m k}$ of the corresponding user-AP pair as $g_{m k}=\sqrt{\beta_{m k}} h_{m k}$. We assume that the entries of $h_{m k}$ are independent and identically distributed (i.i.d) $\mathcal{N}_{\mathbb{C}}(0,1)$ random variables (RVs), and the channels are constant during the coherence interval. 
% %The superscript $(\cdot)^{H}$ means the conjugate-transpose.
% The received pilot signal at $m$-th AP is given by
% \begin{equation}
%     % \mathbf{y}_{m}^{\mathrm{p}}=\sqrt{T } \sum_{k=1}^{K} g_{m k} \boldsymbol{\varphi}_{k}+\mathbf{n}_{m}^{\mathrm{p}},\label{eq:y(SNR)}
%     \mathbf{y}_{m}=\sqrt{\omega N_\mathrm{p}} \sum_{k=1}^{K} g_{m k} \boldsymbol{\varphi}_{k}+\mathbf{n}_{m} \, ,\label{eq:y(SNR)}
% \end{equation}
% where $\omega$ is the normalized transmit signal-to-noise ratio (SNR) of a pilot signal, and $\mathbf{n}_{m}$ is an additive noise vector of the $m$-th AP such that the elements of $\mathbf{n}_{m}$ are i.i.d. $\mathcal{N}_{\mathbb{C}}(0,1)$ RVs.
% The estimate of $g_{mk}$ obtained based on a minimum-mean square error is given by 

% \begin{equation}
%     \hat{g}_{m k}=\frac{\mathbb{E}\left\{\left(\boldsymbol{\varphi}_k^H \mathbf{y}_m\right)^* g_{m k}\right\}}{\mathbb{E}\left\{\left|\boldsymbol{\varphi}_k^H \mathbf{y}_m\right|^2\right\}}\left(\boldsymbol{\varphi}_k^H \mathbf{y}_m\right)=c_{m k}\left(\boldsymbol{\varphi}_k^H \mathbf{y}_m\right),
% \end{equation}
% where
% \begin{equation}
%     c_{m k} \triangleq \frac{\sqrt{N_{\mathrm{p}} \omega} \beta_{m k}}{N_{\mathrm{p}} \omega \sum_{k^{\prime}=1}^K \beta_{m k^{\prime}}\left|\boldsymbol{\varphi}_k^H \boldsymbol{\varphi}_{k^{\prime}}\right|^2+1} \ .
% \end{equation}
% % where the superscript $(\cdot)^{*}$ means the conjugate. 
% From the randomness assumptions for corresponding RVs, the mean-square channel estimate, denoted as $\gamma_{m k}$, is given by

% \begin{equation}
%     %    \gamma_{m k} \triangleq \mathbb{E}\left\{\left|\hat{g}_{m k}\right|^{2}\right\}=\frac{\beta_{m k}^2}{\sum_{k^{\prime}=1}^{K} \beta_{m k^{\prime}}\left|\boldsymbol{\varphi}_{k}^{H} \boldsymbol{\varphi}_{k^{\prime}}\right|^{2}+1/T}\ .\label{eq:mean-sqr channel est}
%     \gamma_{m k} \triangleq \mathbb{E}\left\{\left|\hat{g}_{m k}\right|^{2}\right\}=\frac{N_\mathrm{p}\beta_{m k}^2}{N_\mathrm{p}\sum_{k^{\prime}=1}^{K} \beta_{m k^{\prime}}\left|\boldsymbol{\varphi}_{k}^{H} \boldsymbol{\varphi}_{k^{\prime}}\right|^{2}+1/\omega} \ .\label{eq:mean-sqr channel est}
% \end{equation}
% %If $T \geq K$, then we can choose pairwisely orthogonal pilot sequences $\boldsymbol{\varphi}_{1}, \boldsymbol{\varphi}_{2}, \cdots, \boldsymbol{\varphi}_{K}$ such that $\left|\boldsymbol{\varphi}_{k}^{H} \boldsymbol{\varphi}_{k^{\prime}}\right|^{2}=0$ if $k^{\prime} \neq k$. 
% The orthogonal PA leads to $\left|\boldsymbol{\varphi}_{k}^{H} \boldsymbol{\varphi}_{k^{\prime}}\right|^{2}=0$ if $k^{\prime} \neq k$. The number of users $K$ generally exceeds the number of orthogonal pilot resources $N_\mathrm{p}$, and the same pilot sequences are necessarily reused in the assignment\cite{2017versus, 2018coded}. 
% The quality of the channel estimate $\hat{g}_{m k}$ is degraded by the signal transmitted from a pilot-sharing user $k^\prime$ with $\boldsymbol{\varphi}_{k^{\prime}}=\boldsymbol{\varphi}_{k}$. This induces the pilot contamination. Fig. \ref{fig:1}(a) illustrates a simple example. Two pilot resources are assigned to three users. While AP 1 estimates the channel for user 1, pilot signals from users 2 and 3 interfere due to the pilot reuse.
% % In the uplink payload data transmission, the received signal at the $m$-th AP is given by
% % \begin{equation}
% % y_{m}^{\mathrm{u}}= \sum_{k=1}^{K} g_{m k} s_{k}+n_{m}^{\mathrm{u}},
% % \end{equation}
% % where $s_{k}$ is data symbol of $k$-th user which satisfy $\mathbb{E}\big\{\left|s_{k}\right|^{2}\big\}=1$.
% % $n_{m}^{\mathrm{u}} \sim \mathcal{N}_{\mathbb{C}}(0,1)$ is additive noise at the $m$-th AP.
% % The received signal $y_{m}^{\mathrm{u}}$ and its channel estimate $\hat{g}_{m k}$ are processed into a quantity $\hat{g}_{m k}^{*} y_{m}^{\mathrm{u}}$ by $m$-th AP, and it is transmitted to the CPU through fronthaul link for detection of the symbol $s_{k}$.

% \section{Uplink Payload Data Transmission}

% In uplink payload transmission from users in Fig. \ref{fig:1}(b), all $K$ users simultaneously send their data to the APs, and each AP detects the signals from channel estimates and sends them to the CPU. According to an analysis in \cite{2017versus}, the received signal collected at the CPU can be decomposed into the desired signal (DS) component, the beamforming uncertainty (BU) component, the user interference (UI) component, and noise. Their average powers of $k$-th user are given, respectively, by
% \begin{subequations}
% \begin{align}
%     \mathrm{DS}_{k} =&  ~\omega \eta_{k}\left(\sum\limits_{m=1}^{M} \gamma_{m k}\right)^{2},\\
%     \mathrm{BU}_{k} =&  ~\omega\sum_{k^{\prime}=1}^{K} \eta_{k^{\prime}} \sum_{m=1}^{M} \gamma_{m k} \beta_{m k^{\prime}}  \ ,\\
%     \mathrm{UI}_{k k^{\prime}} =&
%          ~\omega\eta_{k^{\prime}}\left(\sum\limits_{m=1}^{M} \gamma_{m k} \frac{\beta_{m k^{\prime}}}{\beta_{m k}}\right)^{2} \left|\boldsymbol{\varphi}_{k}^{H} \boldsymbol{\varphi}_{k^{\prime}}\right|^{2},\label{eq:contaminationfactor}
% \end{align}
% \end{subequations}
% where $\sqrt{\eta_{k}}$ is a power control coefficient of the $k$-th user, i.e., $\eta_{k} \in (0, 1]$. 
% We assume that the normalized uplink transmit SNR is equal to that of pilot signals, $\omega$.
% Note that \eqref{eq:contaminationfactor} corresponds to the degradation effect of the pilot reuse on an achievable rate of $k$-th user in case of $k\neq k^{\prime}$. The signal to interference and noise ratio (SINR) of $k$-th user and the corresponding achievable rate are given, respectively, by
% \begin{subequations}
% \begin{align}\label{eq:SINR}
%     \mathrm{SINR}_{k} &=
%     \frac{\mathrm{DS}_{k}}{\mathrm{BU}_{k}+\sum\limits_{k^{\prime} \neq k}^{K} \mathrm{UI}_{k k^{\prime}}+\sum\limits_{m=1}^{M} \gamma_{m k}}\ ,\\
%     R_{k} &=\left(1-\frac{N_\mathrm{p}}{N_\mathrm{c}}\right) \log _{2}\left(1+\mathrm{SINR}_{k}\right) \, . \label{eq:achivableRate}
% \end{align}
% \end{subequations}
% %\section{PLACEHOLDER}

% The network throughput maximization is the main purpose of this work. In the next chapter, the PA optimization task is formulated with the achievable rate for each user.
